Source Forager: A Search Engine for Similar Source Code

Developers spend a significant amount of time searching for code: e.g., to understand how to complete, correct, or adapt their own code for a new context. Unfortunately, the state of the art in code search has not evolved much beyond text search over tokenized source. Code has much richer structure and semantics than normal text, and this property can be exploited to specialize the code-search process for better querying, searching, and ranking of code-search results. We present a new code-search engine named Source Forager. Given a query in the form of a C/C++ function, Source Forager searches a pre-populated code database for similar C/C++ functions. Source Forager preprocesses the database to extract a variety of simple code features that capture different aspects of code. A search returns the $k$ functions in the database that are most similar to the query, based on the various extracted code features. We tested the usefulness of Source Forager using a variety of code-search queries from two domains. Our experiments show that the ranked results returned by Source Forager are accurate, and that query-relevant functions can be reliably retrieved even when searching through a large code database that contains very few query-relevant functions. We believe that Source Forager is a first step towards much-needed tools that provide a better code-search experience.

==> tcolorbox.doc.recording.tex <==
% !TeX root = tcolorbox.tex
% include file of tcolorbox.tex (manual of the LaTeX package tcolorbox)
\clearpage
\section{Recording}\label{sec:recording}%
\tcbset{external/prefix=external/recording_}%
The package provides some macros and options to take \emph{records} during
compilation. This is done by \LaTeX\ file operations to save some data
to a file for later usage. The main application scenario is depicted in
\Vref{sec:recording-exercises} where
information about example solutions is recorded and read again
in \Vref{sec:recording-solutions}.

\subsection{Makros}\label{sec:recording-makros}
\begin{docCommand}[doc new=2014-11-28]{tcbstartrecording}{\oarg{file name}}
  Opens a file denoted by \meta{file name} for writing the records.
  The default file name is |\jobname.records|.
  See \Vref{sec:recording-exercises} for an example application.
\end{docCommand}

\begin{docCommand}[doc new=2014-11-28]{tcbrecord}{\marg{content}}
  Records any \meta{content} to the record file.
  \refCom{tcbrecord} is implemented as |\immediate\write|.
  \refCom{tcbstartrecording} has to be called before; otherwise, \refCom{tcbrecord}
  is silently ignored.
\begin{dispListing}
\tcbrecord{\string\solution{\thetcbcounter}{solutions/exercise-\thetcbcounter.tex}}
\end{dispListing}
\end{docCommand}

\begin{docCommand}[doc new=2014-11-28]{tcbstoprecording}{}
  Closes the current record file which was opened by \refCom{tcbstartrecording}
  before.
\end{docCommand}

\begin{docCommand}[doc new=2014-11-28]{tcbinputrecords}{\oarg{file name}}
  Opens a file denoted by \meta{file name} for reading the records via |\input|.
  The default file name is the name of the last used record file for saving.
  \refCom{tcbstoprecording} has to be called before.
\end{docCommand}


\subsection{Options}\label{sec:recording-options}
\begin{docTcbKey}[][doc new=2014-11-28]{record}{=\meta{content}}{style, no default}
  Records any \meta{content} to the record file, see \refCom{tcbrecord}.
  This key can be used several times to write several lines.
  \begin{dispListing}
  record={\string\solution{\thetcbcounter}{solutions/exercise-\thetcbcounter.tex}}
  \end{dispListing}
\end{docTcbKey}

\begin{docTcbKey}[][doc new=2014-11-28]{no recording}{}{}
  Disables \refCom{tcbrecord} and \refKey{/tcb/record} inside the current
  group.
\end{docTcbKey}


\clearpage
\subsection{Example: Exercises}\label{sec:recording-exercises}
The following application example creates exercises and their corresponding
solutions. Each pair is generated inside a single |tcolorbox| where the
solution is given below \refCom{tcblower}. For every example, the solution part
is saved by \refKey{/tcb/savelowerto} to a file. The saving is recorded using
\refKey{/tcb/record}. To enlighten the possibilities, the second exercise
has no solution. Finally, the solutions are input in \Vref{sec:recording-solutions}.

\inputpreamblelisting{L}

\begin{dispListing*}{breakable,before upper=}
\tcbstartrecording

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\sin((\sin x)^2)
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \sin((\sin x)^2) \right)'
    =\cos((\sin x)^2) 2\sin x \cos x.
  \end{align*}
\end{exercise}

\begin{exercise}[no solution]
  It holds:
  \begin{equation*}
    \frac{d}{dx}\left(\ln|x|\right) = \frac{1}{x}.
  \end{equation*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=(\sin(\sin x))^2
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( (\sin(\sin x))^2 \right)'
    =2\sin(\sin x)\cos(\sin x)\cos x.
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\sqrt{x^3-6x^2+2x}
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \sqrt{x^3-6x^2+2x} \right)'
    = \frac{3x^2-12x+2}{2\sqrt{x^3-6x^2+2x}}.
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\left(\frac{2+3x}{1-2x}\right)^3
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \left(\frac{2+3x}{1-2x}\right)^3 \right)'
    = 3 \left(\frac{2+3x}{1-2x}\right)^2 \frac{(1-2x)3-(2+3x)(-2)}{(1-2x)^2}
    = \frac{21(2+3x)^2}{(1-2x)^4}.
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\frac{\cos x}{(\tan 2x)^2}
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \frac{\cos x}{(\tan 2x)^2} \right)'
    = \left( \frac{\cos x (\cos 2x)^2}{(\sin 2x)^2} \right)'\\
    &= \frac{(\sin 2x)^2 [(-\sin x)(\cos 2x)^2+(\cos x)4\cos 2x (-\sin 2x)]
       - \cos x (\cos 2x)^2 4\sin 2x \cos 2x}{(\sin 2x)^4}\\
    &= -\frac{\cos(2x) [\sin x \sin 2x \cos 2x+ 4\cos x(\sin 2x)^2
       + 4 \cos x (\cos 2x)^2]}{(\sin 2x)^3}\\
    &= -\frac{\cos(2x) [\sin x \sin 2x \cos 2x+ 4\cos x]}{(\sin 2x)^3}.
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=\cos((2x^2+3)^3)
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( \cos((2x^2+3)^3) \right)'
    =-\sin((2x^2+3)^3) 3(2x^2+3)^2 2\cdot 2x\\
    &=-12x(2x^2+3)^2\sin((2x^2+3)^3).
  \end{align*}
\end{exercise}

\begin{exercise}
  Compute the derivative of the following function:
  \begin{equation*}
    f(x)=(x^2+1)\sqrt{x^4+1}
  \end{equation*}
\tcblower
  The derivative is:
  \begin{align*}
    f'(x) &= \left( (x^2+1)\sqrt{x^4+1} \right)'
    = 2x\sqrt{x^4+1} + \frac{2x^3(x^2+1)}{\sqrt{x^4+1}}.
  \end{align*}
\end{exercise}

\tcbstoprecording
\end{dispListing*}
\tcbusetemp

\subsection{Example: Solutions}\label{sec:recording-solutions}
This concludes the example given in \Vref{sec:recording-exercises}.
Now, the saved and recorded solutions are included.

\begin{dispListing*}{breakable,before upper=}
\tcbinputrecords
\end{dispListing*}
\tcbusetemp

